Preconditioned Latent Variable Proximal Point Method for Optimal Control Problems with Control Constraints

The latent variable proximal point (LVPP) method solves optimization problems in function spaces with pointwise constraints by a sequence of smooth subproblems whose iterates are strictly feasible. We apply it to linear-quadratic elliptic optimal control problems. Control and observation are distributed but may be restricted to subdomains. We prove that the LVPP subproblems are well posed in appropriate function spaces, that the iteration converges for every sequence of proximity parameters with divergent sum, and that it delivers the Lagrange multiplier of the constraint as a by-product. We interpret the Newton step for the LVPP subproblem as a linear-quadratic optimal control problem with a spatially varying control cost, and we show that Newton's method converges locally quadratically. The Newton systems are solved by the minimal residual method with a block-diagonal preconditioner. We prove that the spectrum of the Newton operator with respect to the inner product defined by the preconditioner is bounded independently of the proximity parameter, the iterate, the mesh and the observation and control domains. The results are combined into a complete algorithm, and tested in numerical experiments.

==> figures/figure-styles.tex <==
% Styles of the figures of Sections 3 and 7, loaded in the preamble by scoop-local.sty.
% The figures of Section 7 are drawn by pgfplots from the CSV files in figures/data when the paper is compiled.
% The CSV files come from the implementation (tools/copy_figure_data.py there); see figures/data/SOURCE.md.
\pgfplotsset{compat=1.18}
\pgfplotsset{table/col sep=comma}
\pgfplotstableset{col sep=comma}

\newcommand{\figdata}{figures/data}   % the folder of the CSV files
\newcommand{\figmeshes}{32,64,128,256}
\newcommand{\figsolutionmesh}{32}     % the final iterate: patch plots of finer meshes exceed the memory of pdflatex
\newcommand{\fighistorymesh}{256}     % the mesh of the history of the minimal residual method

\pgfplotsset{
	every axis/.append style={
		tick label style={font=\scriptsize},
		label style={font=\footnotesize},
		title style={font=\footnotesize},
		legend style={font=\scriptsize, draw=none, fill=none},
		legend cell align=left,
	},
}

% Keep only the rows of a table whose column #1 holds the text #2 (for example accepted = True).
\pgfplotsset{
	discard if not/.style 2 args={
		x filter/.append code={
			\edef\tempa{\thisrow{#1}}%
			\edef\tempb{#2}%
			\ifx\tempa\tempb\else\def\pgfmathresult{inf}\fi
		},
	},
}

% One colour and one mark per mesh, the same in every plot: bright for the coarse mesh, dark for the fine one.
\definecolor{figmesh32}{HTML}{A6CEE3}
\definecolor{figmesh64}{HTML}{4292C6}
\definecolor{figmesh128}{HTML}{08519C}
\definecolor{figmesh256}{HTML}{071A3A}
\pgfplotsset{
	mesh32/.style={color=figmesh32, mark=*},
	mesh64/.style={color=figmesh64, mark=square*},
	mesh128/.style={color=figmesh128, mark=triangle*},
	mesh256/.style={color=figmesh256, mark=diamond*},
}

% The Newton iterates of a subproblem: bright for the start, dark from the seventh iterate on; oranges, so that
% nothing is taken for a mesh.
\definecolor{figstepfirst}{HTML}{FDD0A2}
\definecolor{figstepmiddle}{HTML}{F16913}
\definecolor{figsteplast}{HTML}{7F2704}
\pgfplotsset{colormap={newtonsteps}{color=(figstepfirst) color=(figstepmiddle) color=(figsteplast)}}

% The proximity parameters in the two figures of Section 3: greens, bright for the small parameter and dark for
% the large one, so that nothing is taken for a mesh or for a Newton iterate.
\definecolor{figalphasmall}{HTML}{74C476}
\definecolor{figalphamiddle}{HTML}{31A354}
\definecolor{figalphalarge}{HTML}{006D2C}

% The four parts of the residual of the minimal residual method: neither blue (the meshes) nor orange (the Newton
% iterates).
\definecolor{figpartadjoint}{HTML}{009988}
\definecolor{figpartoptimality}{HTML}{EE3377}
\definecolor{figpartstate}{HTML}{999933}
\definecolor{figpartidentification}{HTML}{AA4499}

% The observation domain and the control domain on the state and the adjoint state: thin white lines with a faint
% dark edge, so that they show on the dark and on the white parts of the colormaps.
\tikzset{
	subdomain/.style={draw=white, line width=0.5pt, preaction={draw=black, draw opacity=0.35, line width=1.3pt}},
}
\newcommand{\figsubdomains}{%
	\draw[subdomain] (axis cs:0.125,0.125) rectangle (axis cs:0.25,0.875);
	\draw[subdomain] (axis cs:0.375,0.375) rectangle (axis cs:0.875,0.875);
}

